Equation level matching: An extension of the method of matched asymptotic expansion for problems of wave propagation

We introduce an alternative to the method of matched asymptotic expansions. In the "traditional" implementation, approximate solutions, valid in different (but overlapping) regions are matched by using "intermediate" variables. Here we propose to match at the level of the equations involved, via a "uniform expansion" whose equations enfold those of the approximations to be matched. This has the advantage that one does not need to explicitly solve the asymptotic equations to do the matching, which can be quite impossible for some problems. In addition, it allows matching to proceed in certain wave situations where the traditional approach fails because the time behaviors differ (e.g., one of the expansions does not include dissipation). On the other hand, this approach does not provide the fairly explicit approximations resulting from standard matching. In fact, this is not even its aim, which to produce the "simplest" set of equations that capture the behavior.

==> TheSections/Sec03_WeaklyNonlinearDetonationsOLD.tex <==
% Equation Level Matching (paper input file).
% Section: Example from waves theory: weakly nonlinear detonations
% ======================================================================= 70
%%% OLD (LONG) VERSION
% Detonation waves in reacting gas dynamics exhibit a very complex and
% interesting behavior, which is as yet not fully understood
% \cite{fickett2011detonation,williams1985combustion,Lee-2008}. With the
% aim of furthering the understanding of the phenomena, simple "ad hoc"
% models for detonations have been proposed
% (e.g. \cite{fickett1979detonation,majda1981qualitative}). Even more
% interesting is that simplified models can be rationalized/derived
% using weakly nonlinear asymptotic expansions in the limit of small
% heat release and large activation energy
% \cite{rosales1983weakly,rosales1989diffraction,clavin2002dynamics,faria2015theory}. These
% model allow not only for qualitative understanding, but quantitative
% comparisons as well.  In particular, there has been some recent
% interest on the influence of transport effects (viscosity, thermal
% conductivity, and species diffusion) on the stability of detonations
% \cite{barker2015viscous,romick2015verified,romick2012effect}. Furthermore,
% when these effects are present, other types of waves (roughly in the
% same regime as detonations) are possible -- i.e., fast deflagrations
% \cite{kapila1983asymptotic}. Thus the study of their possible
% interactions with detonations is of interest. For these reasons, and
% others, simplified asymptotic models that incorporate transport
% effects would be of interest --- but do not quite exist, as explained
% next.

% Unfortunately, in the regime of high activation energy, gas-kinetic
% theory arguments can be made that indicate that then transport effects
% are exponentially small compared with the activation energy (see,
% e.g. the discussion in \cite{faria2015theory}). Hence, within the
% context of traditional weakly nonlinear asymptotic expansions, these
% terms are neglected. Of course, one can artificially assume that the
% transport effects are not exponentially small, and thus arrive at
% simplified asymptotic models that incorporate these effects. This is
% the path taken in \cite{RosalesMajda1983wndw,faria2014thesis}. However, this
% approach is physically incorrect, and not entirely satisfactory. We
% believe that, in order to get around this problem, a more powerful
% tool is needed, one that can combine the power of weakly nonlinear
% asymptotic expansions with the method of matched asymptotic
% expansions. It is, in fact, the search for this tool that motivated
% the research in this paper.

% In this section we show how the equation level method can be used to
% address the issue introduced in the prior paragraph. We do so by using
% a simplified set of starting equations (i.e., not quite the
% compressible reacting Navier Stokes equations), and restrict the
% presentation to the 1-D case only. This makes the presentation of how
% the method works, which is the main purpose here, simpler to
% follow. The application to the full reacting Navier Stokes equations,
% in multi-dimensions, is the subject of current/ongoing work, and will
% be published elsewhere.

% \subsection{The mathematical model}

% The example we will consider here is an abstract
% version of the reacting equations for compressible gas dynamics in
% 1-D. Specifically, in adimensional variables:
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{eqnarray}
%  \vec u_t + \left(\vec F \left(\vec u \right)\right)_x & = &
%                                                              \epsilon^2\,\vec W
%     \left(\frac{1}{\epsilon}\,\vec u \/,\,\lambda\right) + \epsilon\,\delta
%     \,\mathcal{D}(\partial_x)\,\vec u\/, \label{SWND:eqn:01}\\
%  \lambda_t + \phi\left(\vec u\right)\,\lambda_x & = & w \left(
%     \frac{1}{\epsilon}\,\vec u\/,\,\lambda\right)\/, \label{SWND:eqn:02}
% \end{eqnarray}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% where
% \begin{itemize}
%  % ---------------------------------------------------------------------- 70
%  \item
%  $\vec u$ is the vector of ``fluid'' conserved densities ---
%  actually, perturbations from a constant ``rest'' state.
%  % \Dmath{\uvec_0 = \vec{0}}.
%  % ---------------------------------------------------------------------- 70
% \item
%  $\vec F$ is the vector of density fluxes, with $\vec F$ a
%  smooth function of the densities.
%  % ---------------------------------------------------------------------- 70
% \item $\lambda$ is a reaction progress variable, $0 \leq \lambda
%     \leq 1$. Here $\lambda = 0$ corresponds the fresh mixture,
%   while $\lambda = 1$ corresponds to the burned products.
%  % ---------------------------------------------------------------------- 70
%  \item
%  $0 < \epsilon \ll 1$ is the inverse of the ``activation energy''
%  (or the square root of the ``heat release'').
%  % ---------------------------------------------------------------------- 70
%  \item 
%  $\delta$ is a small parameter characterizing the transport
%  effects. We assume that $0 < \delta \ll \epsilon^p$ for any
%  $p > 1$ --- or, at least, for some large $p$. The reason
%  for this assumption is explained in the introduction to this section.
%  % ---------------------------------------------------------------------- 70
%  \item 
%  $\phi$ is the ``particle speed''. Hence the operator on the left
%  in equation (\ref{SWND:eqn:02}) is the ``material derivative''.
%  % ---------------------------------------------------------------------- 70
%  \item 
% $\vec W$ are the sources caused by the ``reaction''. They enter the
%  equations multiplied by the ``heat release'' $\epsilon^2$. Note
%  also the sensitive dependence on the fluid variables (high activation
%  energy) via the pre-factor $1/\epsilon$.
%  % ---------------------------------------------------------------------- 70
%  \item 
% $w \geq 0$ is the reaction rate, which vanishes for
% $\lambda=1$ (hence, if $\lambda$ starts below one, it
%  never goes above it).
%  % ---------------------------------------------------------------------- 70
% \item $\mathcal{D}(\partial_x)$ is a linear, constant coefficients,
% second order, diffusion operator. Specifically,
% $\mathcal D(\partial_x) = D\,\partial_x^2$, where $D$ is a square
% diffusion matrix. By this we mean that all the solutions of the
% linearized ($\vec u$ infinitesimal), non-reacting (no $\lambda$),
% problem decay in time --- i.e., solutions proportional to
% $e^{i\,k\,x+\sigma\,t}$, $\sigma = \sigma(k)$ and $k$ real, have
% $\mathbb{R}(\sigma) < 0$. Furthermore, in the long wave number,
% $\epsilon\,\delta\,|k| \ll 1$, $\mathbb{R}(\sigma)$ is
% proportional to $\epsilon\,\delta\,k^2$ at leading order.

%  Note: the definition above of a diffusion matrix may seem overly
%  complicated, but it is motivated by the fluid dynamics case. There
%  $D$ is singular, since there is no mass diffusion, yet all the
%  listed properties apply.
% \end{itemize}

% We will also assume that the \emph{system is strictly hyperbolic}, that
% is: \emph{the square matrix $\nabla \left(\vec F \right)$ has distinct
% real eigenvalues.}\,\footnote{\,For reacting gases $\phi$ is
%    one of the eigenvalues of $\nabla (\vec F)$. However, here we will
%    not use this fact.}
% Further, for $\vec u$ small expand
% % ----------------------------------------------------------------------- 70
% \begin{equation} \label{SWND:eqn:03}
%  \vec F = \vec F_0 + A_1\,\vec u + \vec{A}_2 \left(\vec u\/,\,\vec u\right)
%        + \vec{A}_3 \left(\vec u\/,\,\vec u\/,\,\vec u\right) + \dots
% \end{equation}
% % ----------------------------------------------------------------------- 70
% where $A_1$ is a square matrix,
% $\vec{A}_2$ is a (symmetric) vector valued bilinear function, etc.

% The motivation for the assumed scalings above is as follows: we seek
% for a situation where the nonlinearity is weak (weakly nonlinear
% waves). Because of the reaction terms, such waves are possible only if
% the heat release is suitably small. In addition, in order for the weak
% waves to couple with the reaction, sensitive dependence of the
% reaction terms on the fluid variables is needed. This leads to the
% high activation energy assumption.  High activation energy is a very
% reasonable assumption; in fact most physical detonation waves occur in
% this regime. Small heat release, however, is more debatable
% assumption. Experiments involving detonation waves are usually done in
% tubes, where wall loses due to viscous friction and thermal
% conductivity are substantial. In this case there is a minimum heat
% release below which a self-sustaining detonation wave is not possible.

% \subsection{Weakly nonlinear detonation waves expansion}\label{SWND:sub:WNDW}

% Let $c$ be an eigenvalue of $A_1$ such that
% $c \neq \phi_0 = \phi(\vec{0})$. Let $\vec l$ and $\vec r$
% be left and right eigenvectors of $A_1$ corresponding to $c$,
% normalized by $\vec l \cdot \vec r = 1$. Then we propose a weakly
% nonlinear traveling wave expansion:
% % ----------------------------------------------------------------------- 70
% \begin{equation} \label{SWND:eqn:04}
%  \vec u \sim \epsilon\,\vec u_1(\chi\/,\,\tau)
%             + \epsilon^2\,\vec u_2(\chi\/,\,\tau) + \dots \quad \mbox{and}
%  \quad \lambda \sim \lambda_0(\chi\/,\,\tau) +
%             \epsilon\,\lambda_1(\chi\/,\,\tau) + \dots\/,
% \end{equation}
% %----------------------------------------------------------------------- 70
% where $\chi = x-c\,t$ and $\tau = \epsilon\,t$. We assume that
% the wave moves into the rest state ($\vec u$ vanishes for
% $\chi \to \infty$).
% % ----------------------------------------------------------------------- 70
% Substituting into (\ref{SWND:eqn:01}), and collecting equal powers
% of $\epsilon$, yields
% % ----------------------------------------------------------------------- 70
% \begin{eqnarray}
%  \mathcal O(\epsilon^1):
%  \qquad (A_1-c)\,(\vec u_1)_\chi &=&
%  0\/.  \label{SWND:eqn:05} \\
%  %
%  \mathcal O(\epsilon^2):
%  \qquad (A_1-c)\,(\vec u_2)_\chi &=&
%  - (\vec u_1)_\tau - (\vec{A}_2(\vec u_1\/,\,\vec u_1))_\chi
%  + \vec W(\vec u_1\/,\,\lambda_0)\/. \label{SWND:eqn:06}\\
%  %
%  \dots &=& \dots \nonumber\\
%  %
%  \mathcal O(\epsilon^n):
%  \qquad (A_1-c)\,(\vec u_n)_\chi &=&
%  - (\vec u_{n-1})_\tau - (\vec{N}_n)_\chi + \vec W_{n-2}\/. \label{SWND:eqn:07}
% \end{eqnarray}
% % % ----------------------------------------------------------------------- 70
% Here, in (\ref{SWND:eqn:07}): \quad
% \begin{enumerate*}[label=(\roman*),before=\hspace{-1.6ex}]
% \item $n \geq 2$,
% \item $\vec{N}_n = \sum_{j \geq 2} \;\; \sum_{n_1+\dots+n_j=n}
%   \vec{A}_j\left(\vec u_{n_1}\/,\, \dots \vec u_{n_j}\right)$
%   with $n_q \geq 1$,
% \item $\vec W_q$ is the $q$-th term in the expansion of $\vec W$
%   --- note that $\vec W_q$ depends on $\vec u_1\/,\, \dots
%     \vec u_{q+1}$ and $\lambda_0\/,\,\dots \lambda_q$ only.
% \end{enumerate*}
% Because of the assumption on the size of $\delta$, no dissipative
% terms appear at any order --- or for any order below $\epsilon^{p+2}$
% if $\delta =O(\epsilon^p)$, for some large $p$.

% From the $\mathcal{O}(\epsilon)$ equations we see that we must take
% \begin{align}
%   \label{eq:7}
%   \vec u_1 = \sigma_1 \vec r,
% \end{align}
% where $\sigma_1 = \sigma_1(\chi,\tau)$ is scalar valued. For the
% $\mathcal O(\epsilon^2)$ equations it is convenient to write $\vec u_2
% = \sigma_2 \vec r + \vec v_2$, where $\vec v_2$ is a linear
% combination of the right eigenvectors of $\vec A_1$ with corresponding
% eigenvalue different from $c$, i.e. $\vec l \cdot \vec v_2 = 0$. Then \eqref{SWND:eqn:06} has a solution
% provided that the right hand side is orthogonal to $\vec l$. That is 
% \begin{equation} \label{SWND:eqn:10}
%  (\sigma_1)_\tau + (a\,\sigma_1^2)_\chi =
%  \vec l\cdot\vec W\left(\sigma_1\,\vec r\/,\,\lambda_0\right)\/,
% \end{equation}
% where $a = \vec l \cdot \vec A_2(\vec r, \vec r)$. More generally, at
% any order we take $\vec u_n = \sigma_n \vec r + \vec v_n$, where $\vec
% l \cdot v_n  = 0$ is determined by \eqref{SWND:eqn:07}. Then
% $\sigma_n$ follows from the solvability condition at the next order
% --- the right had side of \eqref{SWND:eqn:07} must be orthogonal to
% $\vec l$ at all orders (see \S \ref{SWND:WNDW:sss:THOE}).

% Finally the expansion for $\lambda$ is governed by
% \begin{eqnarray}
% \mathcal O(\epsilon^0):
%  \qquad (\phi_0-c)\,(\lambda_0)_\chi &=&
%  w\left(\vec u_1\/,\,\lambda_0\right)\/, \label{SWND:eqn:12}\\
%  \dots &=& \dots \nonumber \\
%  \mathcal O(\epsilon^n):
%  \qquad (\phi_0-c)\,(\lambda_n)_\chi &=& - (\lambda_{n-1})_\tau
%  -\sum_{j=1}^n \phi_j\,(\lambda_{n-j})_\chi + w_n\/, \label{SWND:eqn:13}
% \end{eqnarray}
% where the boundary condition $\lambda = 0$ is imposed for $\chi \to
% \infty$ (ahead of the wave). Here, in (\ref{SWND:eqn:13}),
% $\phi_q$ and $w_q$ are the $q$-th terms in the expansions for
% $\phi$ and $w$. Note that $w_n$ involves dependence on
% $\vec u_{n+1}$ and $\lambda_n$ --- this via the terms
% $(\vec u_{n+1} \cdot \text{grad}_u)\,w(\vec u_1\/,\,\lambda_0)$ and
% $\lambda_n\,w_\lambda(\vec u_1\/,\,\lambda_0)$.

% \subsubsection{The higher orders} \label{SWND:WNDW:sss:THOE}
% %
% At the leading order, equations controlling the expansion are
% (\ref{SWND:eqn:10}), and (\ref{SWND:eqn:12}).  Below we describe how
% the higher order controlling equations look like.

% Substitute $\sigma_1 \to \sigma_1 + \Delta\sigma$ and
% $\lambda_0 \to \lambda_0 + \Delta\lambda$ into (\ref{SWND:eqn:10})
% and (\ref{SWND:eqn:12}), where $\Delta\sigma$ and
% $\Delta\lambda$ are infinitesimals. Then $\Delta\sigma$ and
% $\Delta\lambda$ satisfy linear homogeneous equations (with
% coefficients that depend on $\sigma_1$ and $\lambda_0$)
% % ----------------------------------------------------------------------- 70
% \begin{align*}
% \mathcal L\,\vec{\Delta}=\vec{0},
% \end{align*}
% % ----------------------------------------------------------------------- 70
% where $\vec{\Delta}$ is the vector with components
% $\Delta\sigma$ and $\Delta\lambda$. The higher order equations
% are forced versions of this equation,
% $\mathcal L\,\vec{\Delta}_n=\vec{f}_n$,
% where the right hand sides depend on the lower order terms only, and
% $\vec{\Delta}_n$ is the vector with components $\sigma_n$ and
% $\lambda_{n-1}$ ($n \geq 2$).

% \smallskip\noindent
% % ----------------------------------------------------------------------- 70
% Note: in specific examples one can see that these equations can develop
% secularities for either $\chi$ or $\tau$ large. \emph{The
% expansion in this section is, generally, not valid for either
% $\chi = \mathcal O(1/\epsilon)$ or $\tau = \mathcal O(1/\epsilon)$.}

% \subsection{Burgers' shock waves expansion}\label{SWND:sub:BSWE}

% Change variables in (\ref{SWND:eqn:01}--\ref{SWND:eqn:02}), to
% $T = t/\delta$ and $X = x/\delta$. Then
% % ----------------------------------------------------------------------- 70
% \begin{eqnarray}
%  \vec u_T + \left(\vec F \left(\vec u \right)\right)_X & = &
%     \epsilon^2\,\delta\,\vec W \left(\frac{1}{\epsilon}\,\vec u\/,\,\lambda
%     \right) + \epsilon\,\mathcal D(\partial_X)\,\vec u\/, \label{SWND:eqn:14}\\
%  \lambda_T + \phi\left(\vec u\right)\,\lambda_X & = & \delta\,w \left(
%     \frac{1}{\epsilon}\,\vec u\/,\,\lambda\right)\/. \label{SWND:eqn:15}
% \end{eqnarray}
% % ----------------------------------------------------------------------- 70
% We now expand
% % ----------------------------------------------------------------------- 70
% \begin{equation} \label{SWND:eqn:16}
%  \vec u \sim \epsilon\,\vec u_1(\xi\/,\,\mu)
%             + \epsilon^2\,\vec u_2(\xi\/,\,\mu) + \dots \quad\mbox{and}
%  \quad \lambda \sim \lambda_0(\xi\/,\,\mu) +
%             \epsilon\,\lambda_1(\xi\/,\,\mu) + \dots\/,
% \end{equation}
% %----------------------------------------------------------------------- 70
% where $\xi = X-c\,T$ and $\mu = \epsilon\,T$. It is then easy
% to see that
% % ----------------------------------------------------------------------- 70
% \begin{eqnarray}
%   \mathcal O(\epsilon^1):
%   \qquad (A_1-c)\,(\vec u_1)_\xi &=&
%                                     0\/.  \label{SWND:eqn:17}\\
%  %
%   \mathcal O(\epsilon^2):
%   \qquad (A_1-c)\,(\vec u_2)_\xi &=& - (\vec u_1)_\mu -
%  (\vec{A}_2(\vec u_1\/,\,\vec u_1))_\xi + \mathcal
%                                      D(\partial_\xi)\,\vec u_1\/.
%  \label{SWND:eqn:18}\\
%  %
%  \dots &=& \dots \nonumber\\
%  %
%  \mathcal O(\epsilon^n):
%  \qquad (A_1-c)\,(\vec u_n)_\xi &=& - (\vec u_{n-1})_\mu -
%  (\vec{N}_n)_\xi + \mathcal D(\partial_\xi)\,\vec u_{n-1}\/.\label{SWND:eqn:19}
% \end{eqnarray}
% % ----------------------------------------------------------------------- 70
% The solution to these equations follows the same pattern as for
% (\ref{SWND:eqn:05}--\ref{SWND:eqn:07}). We write
% % ----------------------------------------------------------------------- 70
% \begin{equation} \label{SWND:eqn:20}
%  \vec u_1 = \sigma_1\,\vec r \qquad\mbox{and}\qquad
%  \vec u_n = \sigma_n\,\vec r + \vec v_n \;\;\mbox{for}\;\; n \geq 2\/,
% \end{equation}
% % ----------------------------------------------------------------------- 70
% with $\vec l \cdot \vec v_n=0$. Then the $\sigma_n$ are determined
% by the \emph{solvability conditions: the right hand sides in the equations
% above must be orthogonal to} $\vec l$. In particular:
% % ----------------------------------------------------------------------- 70
% \begin{equation} \label{SWND:eqn:21}
%  (\sigma_1)_\mu + (a\,\sigma_1^2)_\xi
%    = \vec l \cdot \mathcal D(\partial_\xi)\,\vec r\,\sigma_1
%    = \nu\,(\sigma_1)_{\xi\/\xi}\/,
% \end{equation}
% % ----------------------------------------------------------------------- 70
% where $a$ is as in (\ref{SWND:eqn:10}) and
% $\nu = \vec l\cdot D\,\vec r > 0$ is a constant ($\nu > 0$
% follows because $D$ is a diffusion matrix).

% % ----------------------------------------------------------------------- 70
% Note that (\ref{SWND:eqn:21}) \emph{is Burgers'
%   equation},
% the canonical equation describing viscous weak shocks~\cite{burgers1948mathematical,whitham1974linear,choquet1968ondes,hunter1995asymptotic,rosales1991introduction}.

% Similarly
% % ----------------------------------------------------------------------- 70
% \begin{eqnarray}
% \mathcal O(\epsilon^0):
%  \qquad (\phi_0-c)\,(\lambda_0)_\xi &=& 0\/. \label{SWND:eqn:22}\\
%  \dots &=& \dots \nonumber \\
%  \mathcal O(\epsilon^n):
%  \qquad (\phi_0-c)\,(\lambda_n)_\xi &=& - (\lambda_{n-1})_\mu
%  -\sum_{j=1}^n \phi_j\,(\lambda_{n-j})_\xi\/. \label{SWND:eqn:23}
% \end{eqnarray}
% % ----------------------------------------------------------------------- 70
% Note that these equations mean that no reaction occurs in this
% limit.
% % ----------------------------------------------------------------------- 70

% \subsection{Equation level matching} \label{SWND:sub:ELMA}
% %
% Now we extend the process introduced in \S~\ref{sec:asympt-match-equat},
% to the problem in this section. Specifically, consider:
% \begin{enumerate}[label=(\alph*)]
% \item The expansion in \S~\ref{SWND:sub:WNDW}, given by equations
%     (\ref{SWND:eqn:05}--\ref{SWND:eqn:07}) and
%     (\ref{SWND:eqn:12}--\ref{SWND:eqn:13}).
%   \item The expansion in \S~\ref{SWND:sub:BSWE}, given by equations
%     (\ref{SWND:eqn:17}--\ref{SWND:eqn:19}) and
%     (\ref{SWND:eqn:22}--\ref{SWND:eqn:23}).
% \end{enumerate}
% Then take the union of these expansions to produce a unified expansion
% which reduces to those in \S~\ref{SWND:sub:WNDW} and
% \S~\ref{SWND:sub:BSWE} in the appropriate set of variables. That is,
% matching occurs at the equation level. Hence, because the equations match,
% we know that the solutions will also match (in the sense of standard
% matched asymptotic expansions), without the need to actually compute (or
% even know) the solutions.

% % ----------------------------------------------------------------------- 70
% Thus we propose the unified expansion
% % ----------------------------------------------------------------------- 70
% \begin{eqnarray}
%  \vec u & \sim & \epsilon\,\underbrace{\left(
%        \sigma_1(\chi\/,\,\tau\/;\,\delta)\,\vec r\right)}_{\vec u_1} +
%        \epsilon^2\,\underbrace{\left(
%        \sigma_2(\chi\/,\,\tau\/;\,\delta)\,\vec r +
%        \vec v_2(\chi\/,\,\tau\/;\,\delta)\right)}_{\vec u_2} + \dots
%        \label{SWND:eqn:24}\\
%  \lambda & \sim & \lambda_0(\chi\/,\,\tau\/;\,\delta) +
%             \epsilon\,\lambda_1(\chi\/,\,\tau\/;\,\delta) + \dots\/,
%        \label{SWND:eqn:25}
% \end{eqnarray}
% % ----------------------------------------------------------------------- 70
% where $\vec l \cdot \vec v_n = 0$. \emph{Here, unlike
% (\ref{SWND:eqn:04}), or (\ref{SWND:eqn:16}), each of the terms includes
% an explicit dependence on the small parameter $\delta$. Hence a
% term by term formal expansion is not possible. The equations must be
% obtained via matching, as follows:} 
% % ----------------------------------------------------------------------- 70
% \begin{eqnarray}
%  (A_1-c)\,(\vec u_1)_\chi &=& 0\/.  \label{SWND:eqn:26}\\
%  %
%  (A_1-c)\,(\vec u_2)_\chi &=& - (\vec u_1)_\tau -
%     (\vec{A}_2(\vec u_1\/,\,\vec u_1))_\chi +
%     \vec W(\vec u_1\/,\,\lambda_0)  +
%     \delta\,\mathcal D(\partial_\chi)\,\vec u_1\/. \label{SWND:eqn:27}\\
%  %
%  \dots &=& \dots \nonumber\\
%  %
%  (A_1-c)\,(\vec u_n)_\chi &=& - (\vec u_{n-1})_\tau - (\vec{N}_n)_\chi +
%     \vec W_{n-2} + \delta\,\mathcal D(\partial_\chi)\,\vec u_{n-1}\/.
%     \label{SWND:eqn:28}
% \end{eqnarray}
% % ----------------------------------------------------------------------- 70
% Here we use the same notation introduced in \S~\ref{SWND:sub:WNDW} and
% \S~\ref{SWND:sub:BSWE}. Similarly
% % ----------------------------------------------------------------------- 70
% \begin{eqnarray}
%  (\phi_0-c)\,(\lambda_0)_\chi &=& w\left(\vec u_1\/,\,\lambda_0\right)\/.
%     \label{SWND:eqn:29}\\
%  \dots &=& \dots \nonumber \\
%  (\phi_0-c)\,(\lambda_n)_\chi &=& - (\lambda_{n-1})_\tau
%  -\sum_{j=1}^n \phi_j\,(\lambda_{n-j})_\chi + w_n\/. \label{SWND:eqn:30}
% \end{eqnarray}
% % ----------------------------------------------------------------------- 70
% This expansion matches the one in \S~\ref{SWND:sub:WNDW}
% because\,\footnote{Recall that $\delta$ is smaller than any power of
%   $\epsilon$.}  the effect of the terms multiplied by $\delta$ in the
% equations occurs beyond all the $\vec u_n$ and $\lambda_n$,
% so that the equations reduce to those in
% (\ref{SWND:eqn:05}--\ref{SWND:eqn:07}) and
% (\ref{SWND:eqn:12}--\ref{SWND:eqn:13}).
% % ----------------------------------------------------------------------- 70
% On the other hand, rewriting the equations in terms of the variables
% $\xi = \chi/\delta$ and $\mu = \tau/\delta$, it is easy to
% see (same argument) that the expansion here matches the one in
% \S~\ref{SWND:sub:BSWE} --- the equations reduce to those in
% (\ref{SWND:eqn:17}--\ref{SWND:eqn:19}) and
% (\ref{SWND:eqn:22}--\ref{SWND:eqn:23}).

% % % ----------------------------------------------------------------------- 70
% Finally, note that \emph{the leading order uniform expansion is given by}
% % ----------------------------------------------------------------------- 70
% \begin{eqnarray}
%  (\sigma_1)_\tau + (a\,\sigma_1^2)_\chi &=&
%  \vec l\cdot\vec W\left(\sigma_1\,\vec r\/,\,\lambda_0\right) +
%  \nu\,\delta\,(\sigma_1)_{\chi\/\chi}\/, \label{SWND:eqn:31}\\
%  (\phi_0-c)\,(\lambda_0)_\chi &=&
%  w\left(\vec u_1\/,\,\lambda_0\right)\/.
%  \label{SWND:eqn:32}
% \end{eqnarray}
% % ----------------------------------------------------------------------- 70
% Note that the equations in~ \cite{RosalesMajda1983wndw} reduce to the ones
% above for the plane-waves case. However, in~\cite{RosalesMajda1983wndw} the
% non-physical assumption $\delta \sim \epsilon$ was introduced.
% \begin{remark}\label{SWND:rem:02}
%  Unlike the situation in {\rm \S~\ref{SEIM::SBVP:sss:EqMa}},
%  the matching process here does not involve re-expansion/re-summation of
%  the terms in one expansion to obtain the other. This simplification is
%  a result of the assumption (physical fact) that $\delta$ is
%  smaller than any power of $\epsilon$. Else, given that this
%  problem is nonlinear, the matching process would have been much more
%  complicated --- and, quite likely, undoable beyond a few terms.
%  % ---------------------------------------------------------------------- 70
%  In particular, if $\delta = \epsilon^p$ (some $p$ large),
%  the calculations in this whole section \S~\ref{sec:SWND} are correct up
%  to the level of $\vec u_{p+2}$, beyond which the equations must be
%  modified. We will not consider this case here, since there is not much
%  point in going beyond (\ref{SWND:eqn:31}--\ref{SWND:eqn:32}).

%  % ---------------------------------------------------------------------- 70
%  Note that:
%  \begin{enumerate*}[label=(\roman*),before=\hspace{-0.6ex}]
%  \item  The objective of an expansion of this type is, generally, just the
%    leading order term --- which provides the simplest canonical model
%    incorporating the required physics. Hence not being able to carry the
%    matching process beyond a few terms is not a real problem.
%  \item This issue is not particular to this method. Standard matching is
%    also complicated for nonlinear problems, and cannot be carried out
%    beyond a few terms.
%  \end{enumerate*}
% \end{remark}
% % ----------------------------------------------------------------------- 70
% \subsection{Discussion} \label{SWND:sub:DISC}
% %
% We will use here (\ref{SWND:eqn:31}--\ref{SWND:eqn:32}) as an example
% template to discuss the question: 
% % ----------------------------------------------------------------------- 70
% \begin{equation}\label{SWND:eqn:33}
%  \parbox{0.8\textwidth}{\emph{What are the advantages, if any, resulting
%    from being able to incorporate} (in a consistent and rational manner)
%    \emph{higher order terms into the asymptotic governing equations?}}
% \end{equation}
% % ----------------------------------------------------------------------- 70
% \\However, first, a few disclaimers \vspace*{-0.4em}
% %
% \begin{enumerate}[label=(\alph*)]
%  %
%  \item
%  The system in (\ref{SWND:eqn:31}--\ref{SWND:eqn:32}) is too simple, and
%  there are no significant advantages that we know of. The only effect
%  that the dissipative term introduces is to give a structure to the
%  shocks, which in the inviscid case are just point discontinuities moving
%  in space-time. Thus, we will use (\ref{SWND:eqn:31}--\ref{SWND:eqn:32})
%  as a template for the discussion, but the advantages do not actually
%  apply to it. Proviso: If the viscous term is large enough,
%  (\ref{SWND:eqn:31}--\ref{SWND:eqn:32}) exhibits
%  weak-detonations~\cite{RosalesMajda1983wndw}; however these occur in a
%  regime that is rarely achieved for realistic physical values for the
%  parameters.
%  %
%  \item
%  In terms of numerical solutions (\ref{SWND:eqn:31}--\ref{SWND:eqn:32}) is
%  simpler than the original system, but only by a modest factor. The main
%  challenge still exists: the presence of the small constant
%  $\nu\,\delta$ means that the solutions still have very thin layers,
%  which are numerically costly to resolve.
%  %
%  % \item
%  % There is, of course, the satisfaction of tackling a challenge: Can a
%  % method be developed to do tasks like (\ref{SWND:eqn:33})? With the
%  % standard question and answer: Why? Because it is there!
% \end{enumerate}
% % ----------------------------------------------------------------------- 70
% %
% % ----------------------------------------------------------------------- 70
% Given this, let us now discuss some objections, as well as potential
% advantages \vspace*{-0.4em} \improvement{This is very poorly explained
% below. I am not sure what you wanted to say, but I dont think it came
% out clear at all! We have work on this.} 
% %
% \begin{enumerate}[label=(\alph*)]
%  %
%  \item
%  The extra terms can trigger new types solutions. For example, if one
%  adds some more physics into this problem, the resulting equations not
%  only support detonations, but fast deflagrations~\cite{fariaICDERS2015dissipative}
%  as well. Thus the possible interactions between these two types of waves
%  can be studied (work in progress).
%  %
%  \item
%  At least for this example, a standard matching process can be used to
%  add the shocks (as given by \S~\ref{SWND:sub:BSWE}) to the reacting gas
%  structures in \S~\ref{SWND:sub:WNDW}. So, why not just do this in all
%  cases? See items~??, ??, and ??.
%  %
%  \item
%  In answer to the previous item. One reason is that a standard matching requires
%  detailed knowledge of the solutions involved, which may not be available.
%  An example of this occurs with the higher dimensional versions of
%  (\ref{SWND:eqn:31}--\ref{SWND:eqn:32}), where wave focusing or oblique
%  interactions between waves can happen. Even in the inert case this is
%  a topic where the exact nature of what happens near shock intersections
%  is still not fully understood~\cite{Ben-Dor1992,colella1990neumann,%
%  Skews2005, sturtevant1976focusing,tabak1994focusing,TesdallHunter2002,%
%  vonNeumann1943oblique,vonNeumann1943refraction,zakharian2000neumann}.
%  For weak shocks the issue goes back to
%  von Neumann~\cite{vonNeumann1943oblique,vonNeumann1943refraction},
%  who noticed some inconsistencies in the theory for Mach triple
%  points~\cite{whitham1974linear}. Experimental and numerical evidence
%  confirms that something ``strange'' happens for near glancing weak shock
%  interactions~\cite{colella1990neumann,Skews2005,sturtevant1976focusing}.
%  Recent theory~\cite{TesdallHunter2002}, developed in the contex of a
%  2-D asymptotic\,\footnote{\sf \,Note that for inert gases, where a high
%     activation energy assumption plays no role, a scaling where viscous
%     dissipation appears at ``the correct order'' is feasible. Hence
%     ``standard'' weakly nonlinear asymptotic analysis is applicable.}
%  model~\cite{tabak1994focusing} (unsteady transonic small disturbance
%  equations), suggests that the inviscid problem develops a very
%  complicated singularity --- which viscosity, pressumably, regularizes
%  in some fashion. In addition, there is evidence (numerical and
%  experimental) that the theory from the asymptotic model does
%  apply to the full system~\cite{Skews2005,zakharian2000neumann}.
%  % %
%  % % ---------------------------------------------------------------------- 70
%  % % Ben-Dor1992, Shock Waves
%  % % Ben-Dor and Takayama
%  % % The Phenomena of Shock Wave Reflection - a Review of Unsolved
%  % %   Problems and Future Research Needs.
%  % %   Generic review, with experiments and theory. Not focused on
%  % %   weak waves.
%  % %
%  % % colella1990neumann, JFM
%  % % Colella and Henderson
%  % % The von Neumann paradox for the diffraction of weak shock waves.
%  % %   Numerical solution of Euler and comparison with experiments.
%  % %
%  % % Skews2005, JFM
%  % % Skews and Ashworth
%  % % The Physical Nature of Weak Shock Wave Reflection.
%  % %   Experiments; claims that the Hunter singularities are there.
%  % %   I am skeptic. They are seeing singularities? Really?
%  % %
%  % % sturtevant1976focusing, JFM
%  % % Sturtevant and Kulkarny
%  % % The focusing of weak shock waves.
%  % %   Experimental study.
%  % %
%  % % tabak1994focusing, Phy. Fluids
%  % % Tabak and Rosales
%  % % Focusing of weak shock waves and the von Neumann paradox
%  % %   of oblique shock reflection.
%  % %
%  % % TesdallHunter2002, SIAM J. Appl. Math.
%  % % Tesdall and Hunter
%  % % Self-similar solutions for weak shock reflection.
%  % %    Their theory of infinitely nested rarefactions, based
%  % %    on numerical calculations with the asymptotic model.
%  % %
%  % % vonNeumann1943oblique,
%  % %   Oblique reflection of shocks.
%  % % vonNeumann1943refraction,
%  % %   Refraction, intersection and reflection of shock waves.
%  % % von Neumann, J.
%  % %
%  % % zakharian2000neumann, JFM,
%  % % Hunter et al.
%  % % The von Neumann paradox in weak shock reflection.
%  % %   Solve Euler numerically.
%  % %   Claim agreement with numerics on asymptotic model.
%  % % ---------------------------------------------------------------------- 70
%  % %
%  \item
%  % Continuing with item~e.
%  Another example is the situation described in
%  item~c. Even with detailed standard matching representations for the two
%  types of wave, how does one study their interactions without having to
%  involve the full system of equations (at which point the advantage of
%  having ``simple'' asymptotic representations for the waves is, mostly,
%  lost)? In general, whenever the aim is to study the dynamics and
%  interactions of various types of objects, having them represented via a
%  standard matching approximation creates difficulties.
%  %
%  \item
%  Continuing with item ??. Another example arises in the context of
%  stability studies, which require a solution to begin with. Stability
%  studies starting from solutions represented via a standard matching
%  approximations are complicated by the fact that one does not have an
%  actual solution. For example, in linearized stability, the aim is to
%  study the behavior of infinitesimal perturbation --- which are, of
%  course, much smaller than the errors in the approximation. There are ways
%  around this issue, but they are not simple. By contrast, in a set-up like
%  (\ref{SWND:eqn:31}--\ref{SWND:eqn:32}), one studies everything within
%  the context of the model~\cite{humpherys2013stability,lyng2004stability}.
%  %
% \end{enumerate}
%
% ----------------------------------------------------------------------- 70
%
% ======================================================================= 70
% EOF
